Mapping of CNNs on multi-core RRAM-based CIM architectures

RRAM-based multi-core systems improve the energy efficiency and performance of CNNs. Thereby, the distributed parallel execution of convolutional layers causes critical data dependencies that limit the potential speedup. This paper presents synchronization techniques for parallel inference of convolutional layers on RRAM-based CIM architectures. We propose an architecture optimization that enables efficient data exchange and discuss the impact of different architecture setups on the performance. The corresponding compiler algorithms are optimized for high speedup and low memory consumption during CNN inference. We achieve more than 99% of the theoretical acceleration limit with a marginal data transmission overhead of less than 4% for state-of-the-art CNN benchmarks.

==> intro.tex <==

In recent years, the broad application of \acp{cnn} yielded an ever-growing demand for more efficient computer architecture to handle these compute- and data-intensive workloads. The massive parallelism and reuse opportunities in \acp{cnn} gave existing architectures novel use cases, like GPUs, or generated novel architectures, like TPUs. All improvements aim to squeeze out the highest possible performance within power and area budgets. Today, specialized architectures for \acp{cnn} are found in all form factors, from power-efficient edge devices to hyper-scaled compute clusters.

Despite the massive innovation sparked by the ubiquitous use of \acp{cnn}, all these custom architectures suffer from one major performance limitation: Moving data from the system's main memory to the compute units, and vice versa, as shown in the roof-line plots \cite{jouppi2017datacenter}. In other words, \ac{cnn} accelerators suffer from a von Neumann bottleneck.

\begin{figure}[htbp]
    \centering
    \includesvg[inkscapelatex=false, width=.8\linewidth, keepaspectratio]{figures/overview.svg}
    \caption{Overview of the tools and the workflow}
    \label{fig:overview}
\end{figure}

Novel memory technologies, such as \ac{rram}, promise to tackle this bottleneck as they enable \ac{cim} architectures \cite{NeuRRAM}. \ac{rram} allows storing a \ac{cnn} weight as a resistance value and performing a matrix-matrix computation using analog computing without moving the value from memory. This capability is achieved by organizing the \ac{rram} cells into a crossbar structure, applying voltages as inputs (for the features), and using Kirchhoff's law to generate an output current. \ac{cim} promises to improve energy efficiency and compute latency, as weights of the \ac{cnn} do not leave the memory. 

Many computer architectures have been proposed using these matrix-matrix multiply memories as compute elements for \acp{cnn} \cite{NeuRRAM, ankit2019puma, chi2016prime}, offering unprecedented power efficiency. These architectures generally follow a hierarchical design to scale from a small crossbar (limited by physical constraints) to a whole system executing a \ac{cnn}. Multiple crossbars are arranged into larger matrix-vector processors (e.g., the MVMU from PUMA \cite{ankit2019puma}). Multiple of these processors are then interconnected to scale to a whole accelerator. As the \ac{cim} scheme targets a weight-stationary data flow in which neurons are statically mapped to individual memory cells, large distributed multi-core \ac{cim} accelerators are the standard system architecture.

As for any multi-core system, efficient synchronization is essential for a high-performance system design, which has not been researched sufficiently so far for \ac{cim} systems. Several techniques are researching how to map a convolutional layer (Conv2D) to multiple matrix-vector multiplications. In most cases, im2col is used as it is the simplest and also the most memory efficient in terms of \ac{rram} crossbar memory. However, input data reuse for a single crossbar architecture can also be targeted [Y]. The exchange of partial results between crossbars is usually not considered in previous works, which is highly unrealistic and a significant bottleneck. Only PUMA includes a synchronization technique in HW and SW, but [name 1-2 downfalls for their approach].

